Synthetic Sandbox for Training Machine Learning Engineering Agents

As large language model agents advance beyond software engineering (SWE) tasks toward machine learning engineering (MLE), verifying agent behavior becomes orders of magnitude more expensive: while SWE tasks can be verified via fast-executing unit tests, MLE verification requires running full ML pipelines -- data preprocessing, model training, and metric evaluation -- on large datasets at each rollout step, rendering trajectory-wise on-policy reinforcement learning (RL) prohibitively slow. Existing approaches retreat to supervised fine-tuning (SFT) or offline proxy rewards, sacrificing the exploration and generalization benefits of on-policy RL. We observe that sandbox data size is the primary source of this bottleneck. Based on this insight, we introduce SandMLE, a multi-agent framework that generates diverse, verifiable synthetic MLE environments from a small number of seed tasks, preserving the structural and technical complexity of real-world problems while constraining datasets to micro-scale (each task is paired with only 50-200 training samples). Through extensive experiments, we show that SandMLE reduces execution time by over 13 times, enabling large-scale, on-policy trajectory-wise RL for the first time in the MLE domain. On MLE-bench-lite, SandMLE yields significant gains over SFT baselines across Qwen3-8B, 14B, and 30B-A3B, with relative medal rate improvements ranging from 20.3% to 66.9%. Furthermore, the trained policy generalizes across unseen agentic scaffolds, achieving up to 32.4% better HumanRank score on MLE-Dojo.

==> colm_sections/0_abstract.tex <==
% As LLM agents advance beyond software engineering (SWE) toward machine learning engineering (MLE)---tasks requiring iterative data analysis, model development, and experimental evaluation---training these agents via on-policy reinforcement learning (RL) becomes both an urgent priority and a critical bottleneck.
%
% Unlike SWE tasks, MLE environments require executing full ML pipelines on large datasets at each rollout step, making trajectory-wise RL prohibitively slow.
%
As large language model (LLM) agents advance beyond software engineering (SWE) toward machine learning engineering (MLE), verifying agent behavior becomes orders of magnitude more expensive: while SWE tasks can be verified via fast-executing unit tests, MLE verification requires running full ML pipelines---data preprocessing, model training, and metric evaluation---on large datasets at each rollout step, rendering trajectory-wise on-policy reinforcement learning (RL) prohibitively slow.
%
Existing approaches retreat to supervised fine-tuning (SFT) or offline proxy rewards, sacrificing the exploration and generalization benefits of on-policy RL.
%
We argue that \textit{sandbox data size} is one of the primary sources of this bottleneck.
%
Based on this insight, we introduce \textbf{\ours}, a framework that automatically generates diverse, verifiable synthetic MLE environments from seed tasks, preserving the structural and mathematical complexity of real-world problems while constraining datasets to micro-scale (50–200 samples).
%
\ours reduces execution time by over 13×, enabling large-scale, on-policy trajectory-wise RL for the first time in the MLE domain.
%
On MLE-bench-lite, \ours yields a 20.3\% to 66.9\% relative improvement in medal rate over the SFT baselines across the Qwen3-8B, 14B, and 30B-A3B.
% \zz{may check back later to see if we want to claim a x\% - y\% improvement across different scaffolds}
%
Furthermore, the trained policy generalizes across unseen agentic scaffolds, achieving up to 32.4\% relative improvement in HumanRank score on MLE-Dojo.
% \zz{I see that we have big improvement on human rank socre, why dont we use that?}
% \yf{what's the untrained number?}

==> colm_sections/1_introduction.tex <==
\section{Introduction}
\label{sec:intro}

Large Language Models (LLMs) have demonstrated exceptional reasoning capabilities, particularly when optimized through Reinforcement Learning with Verifiable Rewards (RLVR)~\citep{guo2025deepseek}.
%
However, as these models are deployed to solve increasingly complex problems, machine learning engineering (MLE) has emerged as a challenging frontier.
%
Unlike simple question answering, MLE tasks inherently cannot be resolved in a single turn; they require an agent to iteratively propose ideas, write code, execute it, analyze environment feedback, and adjust its strategy over multiple attempts.
%
Most existing work on applying LLM agents to MLE tasks focuses on developing complex agent scaffolding to improve task performance~\citep{toledo2025ai, liu2025ml}, but these framework-level enhancements do not fundamentally improve the agent's intrinsic reasoning abilities.
%

For similar long-horizon challenges, such as software engineering (SWE)~\citep{jimenez2024swebench} and web search~\citep{zhou2023webarena}, previous works have successfully utilized trajectory-wise reinforcement learning (RL) to enhance LLM reasoning~\citep{wu2025webdancer, deepswe2025, wu2025resum, chen2025scaling}.
%
This training paradigm extends rollouts across multiple turns, assigning rewards based on the final outcome of the trajectory to optimize the model's long-horizon decision-making capabilities.
%
In SWE tasks, unit tests execute in seconds; while in MLE, a single code execution may require training a model from scratch.
%
This orders-of-magnitude gap in feedback latency makes applying online RL to MLE a critical bottleneck: each rollout step requires executing full ML pipelines---data preprocessing, model training, and metric evaluation---with a single code execution averaging nearly 200 seconds on standard problems.
%
% However, applying online RL to MLE introduces a critical bottleneck: each rollout step requires executing full ML pipelines---data pre-processing, model training, and metric evaluation---making environment feedback prohibitively slow.
%
This computational overhead renders the large-scale rollouts required for trajectory-wise RLVR highly impractical.
%
% The computational overhead required to process data, train baseline models, and evaluate metrics makes the large-scale rollouts required for trajectory-wise RLVR highly impractical.
%
Consequently, the few existing efforts that do attempt to train models for these MLE tasks have largely retreated to supervised fine-tuning (SFT) or step-wise RLVR using proxy offline rewards~\citep{cai2026acegrpo, liu2025mlagent}, sacrificing the exploration and generalization benefits typically achieved through on-policy algorithms like Group Relative Policy Optimization (GRPO)~\citep{shao2024deepseekmath} and others~\citep{chu2025sft, zhou2025disco, yu2025dapo, yang2025let}.
%


A closer analysis reveals a surprisingly simple root cause.
%
Unlike SWE, where execution time is dominated by compilation and test logic, MLE latency is overwhelmingly driven by dataset size.
%
% Compared to standard SWE tasks, we observe that the primary driver of execution latency in MLE is the size of the underlying datasets.
%
Based on this insight, we introduce \ours (\figref{fig:teaser}), a novel paradigm that utilizes multi-agent collaboration to generate synthetic MLE sandboxes where training and test data are intentionally constrained to micro-scale (50-200 samples), reducing average execution time to under 15 seconds and enabling thousands of on-policy rollout updates where previously only a handful were feasible.
% data, 
% which is then used to perform trajectory-wise GRPO.
%
For the data construction pipeline of \ours, we design a fully-automated, agent-driven framework that generates diverse, verifiable MLE tasks.
%
By drastically reducing the data volume while preserving the structural complexity and mathematical hidden rules of the machine learning (ML) problem, \ours facilitates high-speed environment feedback, making large-scale, online rollouts practical.
%

Specifically, our pipeline orchestrates multiple specialized agent roles (\figref{fig:syntho_diagram}): 
a \textit{Data Strategist} abstracts the structural DNA from seed tasks to formulate novel scenarios; 
an \textit{MLE Developer} procedurally generates the raw data assets;
an \textit{MLOps Engineer} constructs deterministic evaluation sandboxes with established performance thresholds;
and a \textit{Technical Writer} synthesizes the final task specifications.
%
Using this generated synthetic data, we apply a specifically designed reward formulation and training pipeline to execute trajectory-wise RL, directly enhancing the model's MLE problem solving capabilities.
%

Our main contributions are summarized as follows:
\begin{itemize}[leftmargin=*]
    \item \textbf{Scalable Synthetic MLE Sandbox Generation:} 
    We design a novel multi-agent framework that procedurally extracts structural DNA from seed tasks to generate diverse, high quality, and verifiable synthetic MLE tasks with micro-scale datasets.
    %
    
    \item \textbf{Trajectory-wise RL for MLE:}
    Leveraging these synthetic environments, we propose and successfully apply trajectory-wise RL with the milestone-based reward to the MLE domain, enabling LLMs to learn complex, long horizon trial-and-error strategies.
    %
    
    \item \textbf{Framework-Agnostic Generalization:} 
    Through extensive experiments, we demonstrate that models trained via our approach not only achieve significant performance gains, including a 20.3\% to 66.9\% relative improvement in \texttt{Any Medal} rate over the SFT baseline across various models on MLE-bench-lite~\citep{chan2024mle}, but also generate robustly across unseen agentic scaffolds,
    achieving up to 32.4\% relative improvement in HumanRank score on the MLE-Dojo benchmark~\citep{qiang2025mle}.
    % \zz{need to revisit this bullet point after the experiment section}
    %
\end{itemize}

\begin{figure}[t]
    \centering
    % \includegraphics[width=\linewidth]{figure/teaser_pipeline.png}
    \includegraphics[width=\linewidth]{figure/teaser_updated.png}
    \vspace{-0.25in}
    \caption{
        Standard on-policy RL for MLE tasks (left) is bottlenecked by execution latency: each rollout step requires running full ML pipeline on large associated datasets ($>$200s).
        %
        \ours transforms seed tasks into diverse synthetic environments with micro-scale datasets ($<$15s), making trajectory-wise on-policy RL practically feasible.
        %
        % \zz{3. (just thinking out loud) task, agent that solves the task, training data associated with the task, these three pieces are not completely clear, e.g., laugh/cry LLM has no input (should be the task). But I am guessing these were omitted for brevity and simplicity.}
        % Compared to standard on-policy RL training on real MLE tasks, our \ours framework utilizes an agent pipeline to transform seed tasks into diverse tasks with micro-scale training datasets.
        %
        % This preserves task complexity while reducing execution time to under 15 seconds, enabling highly efficient, trajectory-wise RL.
        }
    \label{fig:teaser}
    \vspace{-0.2in}
\end{figure}

==> colm_sections/2_related.tex <==
% \section{Related Work}
% \label{sec:related}

% \paragraph{Machine Learning Engineering (MLE) for Agents.}

% The rapid advancement in the reasoning capabilities of LLMs has recently enabled their application to complex, open-ended MLE tasks.
% %
% To systematically evaluate these capabilities, MLE-bench~\citep{chan2024mle} was introduced as a major benchmark curating real-world Kaggle competitions with standardized medal-rate evaluation.
% %
% Building on this foundation, MLE-Dojo~\citep{qiang2025mle} and MLE-Smith~\citep{qiang2025mles} have expanded the volume and diversity of available MLE tasks to facilitate broader evaluation.
% %

% Concurrently, substantial research has focused on enhancing agent performance through sophisticated scaffoldings and test-time compute scaling~\citep{nam2025mle}.
% %
% Evolutionary and iterative frameworks, including AIDE~\citep{jiang2025aide}, AIRA~\citep{toledo2025ai}, ML-Master~\citep{liu2025ml, zhu2026toward}, as well as broader systems like the R\&D Agent~\citep{yang2025r} and FM Agent~\citep{li2025fm}, leverage multi-turn environmental feedback to iteratively refine their reasoning trajectories at inference time. 
% %
% While these approaches effectively improve task performance, the gains are contingent on specific scaffold design rather than the underlying model's reasoning capacity.
% % they do not fundamentally improve the intrinsic reasoning abilities of the underlying base models. 
% %
% Indeed, our own cross-framework evaluation (\tabref{tab:generalization_lite},~\ref{tab:generalization_dojo}) reveals that the same base model can exhibit dramatically different performance depending on the scaffold, underscoring that scaffolding alone does not yield robust, transferable MLE capabilities.
% %
% In contrast to these inference-only approaches, \ours targets this gap directly by enabling scalable on-policy RL training, enhancing the model's intrinsic engineering reasoning in a framework-agnostic manner.
% % approach enables scalable RL for on-policy training, directly enhancing the model's fundamental engineering capabilities.
% %

% \paragraph{Reinforcement Learning for MLE Agents.}
% \label{subsec:rl_mle_agents}

% % Agentic reinforcement learning transitions large language models from static text generators to learnable policies operating within sequential decision loops~\citep{zhang2025landscape, singh2025agentic}. 
% Recent works~\citep{zhang2025landscape, singh2025agentic} have demonstrated that execution-based, trajectory-wise RL can effectively optimize agents for long-horizon tasks.
% %
% DeepSWE~\citep{deepswe2025} and WebDancer~\citep{wu2025webdancer} show strong results in software engineering and web search respectively, while~\citet{chen2025scaling} demonstrate that synthesizing diverse experience trajectories further improves policy learning.
% %
% % DeepSWE~\citep{deepswe2025} demonstrates that execution-based RL effectively optimizes agents for long-horizon software engineering tasks. 
% %
% However, extending these frameworks to MLE introduces a severe computational bottleneck: each rollout step requires training and evaluating ML models to derive environmental rewards renders standard on-policy RL prohibitively slow~\citep{cai2026acegrpo}.
% %

% To bypass this latency, prior approaches have relied on SFT over expert trajectories or utilize asynchronous step-wise RL architectures to hide execution time~\citep{liu2025ml, yang2025reinforcement}. 
% %
% Yet, both strategies are fundamentally off-policy; for instance, asynchronous GRPO relies on trajectories generated from lagging policy states, creating a distribution shift~\citep{cai2026acegrpo}. 
% %
% In contrast, \ours leverages fast-executing synthetic environments to maintain a strictly on-policy training regime. 
% %
% By eliminating the execution bottleneck, we ensure that the accumulated reasoning trajectories are natively generated from the current model state, providing a high-fidelity gradient signal for effective and stable learning.
% %



==> colm_sections/3_prelim.tex <==
\section{Preliminaries}\label{subsec:preliminaries}

% Before introducing our proposed approach, \ours, we first formally define the MLE task as an iterative optimization process and briefly review RLVR.
%

% \subsection{LLMs Iteratively Solve MLE Tasks.}
\subsection{MLE as a Sequential Decision Process}\label{subsec:SDP}
We formalize the MLE task as a sequential decision process and review GRPO~\citep{shao2024deepseekmath}, the RLVR algorithm we employ, along with the specific challenges that arise when applying it to multi-turn agentic settings.
%
Specifically, an MLE task can be defined by a tuple $(I, \mathcal{T}, \mathcal{E})$, where $I$ denotes the initial task specification (dataset description and objective), $\mathcal{T}$ represents the available tool set (e.g., code execution, file I/O, and scoring functions), and $\mathcal{E}$ is the interactive execution environment.
%

We cast the agent's interaction with $\mathcal{E}$ as a finite-horizon sequential decision problem.
%
At each step $t$, the language model policy $\pi_\theta$ observes the current trajectory history $h_t = \{I, \mathcal{T}, a_1, o_1, \dots, a_{t-1}, o_{t-1}\}$, comprising the task specification and all prior action–observation pairs. 
%
Conditioned on $h_t$, the language model policy $\pi_\theta$ generates an action $a_t \sim \pi_\theta(\cdot \mid h_t)$, which typically consists of generating or updating code to construct the ML pipeline.
%
The environment $\mathcal{E}$ then executes the action $a_t$ and returns an observation $o_t$, which may include standard output, runtime errors, or intermediate evaluation metrics, extending the history to $h_{t+1} = h_t \cup \{a_t, o_t\}$. 
%
% The history is subsequently updated as $h_{t+1} = h_t \cup \{a_t, o_t\}$.
%
This iterative loop continues until a termination condition is reached, e.g., the agent emits a designated submission action, or a maximum step limit $T_{\text{max}}$ is reached. 
%
Upon completion, the agent's final output is evaluated against a hidden test set to yield a scalar score $S$; for example, in the Kaggle-style benchmarks~\citep{chan2024mle}, $S$ is derived from the agent's relative ranking on the task leaderboard.
%

\paragraph{The execution-latency bottleneck.}
A fundamental bottleneck in this formulation is the environment execution latency.
%
Unlike unit tests in SWE tasks, MLE tasks inherently require training ML models and performing inference over large datasets, making each environment step orders of magnitude more expensive.
%
% Consequently, obtaining the intermediate feedback $o_t$ is highly time consuming.
%
Because on-policy RL invokes $\mathcal{E}$ at every step of every rollout for every sample in a group, this latency renders optimization prohibitively expensive.
%
Prior work has therefore typically permitted extended time windows of up to 24 hours for an agent to complete a single task~\citep{toledo2025ai, liu2025ml}.
%

\subsection{Reinforcement Learning from Verifiable Rewards (RLVR)}\label{subsec:rlvr}

RLVR leverages objective, rule based feedback to optimize LLMs.
%
GRPO~\citep{shao2024deepseekmath} is an efficient variant of Proximal Policy Optimization~\citep{schulman2017proximal} that eliminates the need for an independent value network.
%
Instead, GRPO evaluates the relative quality of responses within a specifically sampled group.
%
For a given input query $x$, the old policy $\pi_{\text{old}}$ samples a group of $N$ candidate outputs $\{y_1, y_2, \dots, y_N\}$.
%
Each candidate output receives a verifiable reward $r_i$ from the environment.
%
The advantage $\hat{A}_i$ for each specific output is computed by normalizing the rewards strictly within the sampled group: 
$ \hat{A}_i = \frac{r_i - \mu_r}{\sigma_r}, $
where $\mu_r$ and $\sigma_r$ are the mean and standard deviation of the group rewards.
%
The GRPO objective maximizes this relative advantage while simultaneously penalizing the KL divergence from a reference model $\pi_{\text{ref}}$ to prevent policy collapse:
%
\begin{equation}
    J_{\text{GRPO}}(\theta) = \mathbb{E}_{x \sim P, y_i \sim \pi_{\text{old}}} \left[ \frac{1}{N} \sum_{i=1}^N \min \left( \rho_i \hat{A}_i, \text{clip}(\rho_i, 1-\epsilon, 1+\epsilon) \hat{A}_i \right) - \beta \mathbb{D}_{\text{KL}}(\pi_\theta \| \pi_{\text{ref}}) \right]
    \nonumber
\end{equation}
%
where $\rho_i = \frac{\pi_\theta(y_i|x)}{\pi_{\text{old}}(y_i|x)}$ is the probability ratio, $\epsilon$ is the surrogate clipping threshold, and $\beta$ is the coefficient controlling the KL penalty.
%

% \paragraph{From step-wise to trajectory-wise RL.}
\paragraph{Applying GRPO to multi-turn, trajectory-level agentic tasks.}
GRPO is agnostic to the internal structure of each output $y_i$, i.e., the algorithm itself is unchanged whether $y_i$ is a single-turn response or a multi-turn trajectory.
%
In the agentic MLE setting, each $y_i$ is no longer a single model generation but a trajectory $\tau_i = \{a_1, o_1, \dots, a_T, o_T\}$ in which model-generated actions $a_t$ alternate with environment-generated observations $o_t$, and the policy gradient is computed only over action tokens while masking observations from the loss~\citep{deepswe2025, wu2025webdancer}.
%
This multi-turn structure introduces two practical challenges that make naive application difficult.
%
First, \textit{reward sparsity}: unlike single-turn RLVR (e.g., math or QA), where reward is available immediately after generation, the agentic reward $r_i$ is determined only upon trajectory completion, after potentially dozens of action-observation exchanges, making credit assignment substantially harder. 
%
Second, \textit{execution cost}: each rollout step invokes the environment $\mathcal{E}$, and each trajectory is sampled $N$ times per input for group normalization, so the total wall-clock cost scales as $O(N \cdot T_{max} \cdot c_{exec})$ per training example.
%
When $c_\text{exec}$ is on the order of minutes, as in standard MLE benchmarks, on-policy training becomes infeasible.
%
Our approach addresses both two challenges directly: \ours reduces $c_\text{exec}$ by over $13\times$ through synthetic micro-scale environments (\secref{subsec:synthetic_pipeline}), and we design a dense, milestone-based reward to mitigate sparsity (\secref{subsec:trajectory_grpo}).


% In traditional step-wise reinforcement learning, LLMs generate a complete response $y$ in a single turn, and the environment immediately provides the reward $r_i$ based on that one shot generation.
%
% However, with the recent development of agentic reinforcement learning for complex domains~\citep{deepswe2025, wu2025webdancer}, this single turn formulation is insufficient.
%
% For trajectory-wise RLVR, the LLM must interact with the environment over multiple sequential turns, accumulating a history of actions and observations to form a complete computational trajectory $\tau_i = \{a_1, o_1, \dots, a_T, o_T\}$. 
%
% In this expanded setting, the verifiable reward $r_i$ is typically sparse and only obtained at the final step based on the overall success of the entire interaction. 
%
% The trajectory-wise GRPO algorithm thus applies the final group relative advantage $\hat{A}_i$ to the entire sequence of generated actions, optimizing the LLM to effectively navigate long horizon interactions and compounding decisions.

==> colm_sections/4_method.tex <==
\section{\ours Framework}\label{sec:workflow}
To enable computationally feasible trajectory-wise RL for MLE, we must first overcome the prohibitive execution latency of real-world tasks.
%
While downsampling datasets seems like a natural solution, it fundamentally corrupts the evaluation environment by breaking fixed test sets and invalidating established leaderboard baselines.
%
Furthermore, downsampling alone does not address the scarcity of diverse training tasks required for robust policy optimization.
%
To address these limitations, we propose \ours, a framework that algorithmically generates a massive, diverse curriculum of synthetic MLE tasks with their associated data and environment.
%
By constructing these sandboxes from the ground up at a micro-scale, we ensure that the entire pipeline---from preprocessing to inference---executes in a fraction of the time. 
%
This strategic reduction preserves the integrity of the reward signal while scaling the number of unique training environments, transforming GRPO into a feasible on-policy training paradigm for MLE agents.
%
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/diagram_syntho.png}
    \vspace{-0.2in}
    \caption{
    % \zz{
    % what we want to show off in this diagram:
    % 1. Bottleneck
    % (a) Existing task (seed task) contains huge associated training data.
    % (b) seed task has much less variance
    % 2. High level
    % (a) One to Many
    % (b) Big to small
    % }
        The Agentic MLE Environment Factory.
        % \zz{We may want to clear up the namings a little bit. The start of this section and the pipeline overview can give readers an impression that \ours == MLE env generation pipeline. But then it also seems to mean that \ours == MLE env generation pipeline (The Agentic MLE Environment Factory) + Trajectory GRPO).}
        %
        Illustrated is the procedural multi-agent workflow that transforms a massive, slow-executing seed task into a coherent, high-speed, verifiable \textit{synthetic micro-task}.
        %
        The pipeline explicitly optimizes for data efficiency by strictly controlling the task-associated training data size (down from 196,157 to less than 200) to enable rapid iteration during policy optimization.
        %
        % \zz{I think the flow is a bit hard to follow, from the figure I don't seem to get that Data Strategist -$>$ MLE Developer -$>$ MLOps Engineer -$>$ Technical Writer. Also the boxes seem to be inconsistent in terms of sizes and fonts.}
    }
    \label{fig:syntho_diagram}
    \vspace{-0.2in}
\end{figure*}
%


\subsection{Synthetic Environment Generation}\label{subsec:synthetic_pipeline}
\paragraph{Pipeline overview.}
As illustrated in \figref{fig:syntho_diagram}, our automated road map transforms curated seed tasks into lightweight synthetic environments through four interconnected phases:
% 1. \textit{Task Amplification and Specification}: An agent extracts the structural blueprint of a real-world seed task, alters its application domain, and defines underlying mathematical rules and noise distributions;
% 2. \textit{Agentic Data Generation}: A code-driven approach is employed to procedurally generate the small-scale datasets, applying the hidden rules to establish ground truth labels; 
% 3. \textit{Evaluation Environment Setup}: We construct an automated sandbox to safely execute the policy's generated code and calculate final metrics against a hidden test set; 
% 4. \textit{Task Description Synthesis}: Finally, the original seed task's narrative is adapted to precisely match the newly generated domain and feature schema, ensuring an accurate prompt for policy optimization.
1. \textit{Task Amplification and Specification};
2. \textit{Agentic Data Generation}; 
3. \textit{Evaluation Environment Setup}; 
and 4. \textit{Task Description Synthesis}.
%
We illustrate each components with details next.
%
Prompt templates for all pipeline stages are detailed in \appref{sec:prompt}.


\paragraph{Data Strategist: Seed Task Amplification and Specification.}
\label{subsec:task_amplification}
To maximize the diversity of our synthetic environments, a \textit{Data Strategist} agent extracts and manipulates the core structure of real-world seed tasks through four steps: 
(i) \textit{Structural DNA Extraction}: the agent abstracts a seed task into a \textit{Task DNA}, which is a mathematical schema (e.g., modality, resolution, label cardinality) stripped of semantic context.
%
(ii) \textit{Domain Attribution}: the abstracted DNA is then mapped to broader scenarios (e.g., re-purposing an animal image classification into road damage detection).
%
(iii) \textit{Adversarial Mutation}: the agent injects realistic difficulty via a noise configuration $\epsilon$ (e.g., image blurring).
%
% And (iv) \textit{Concrete Specification Compilation}: the agent merges these elements, defining a complex hidden rule $H: l = f(z) + \epsilon$
% \zz{not sure if I actually understand what "hidden rule" means, can we show an example here?}
% that connects individual features $z$ to labels $l$ in the synthetic micro dataset $Z$, while restricting the total dataset size to 50--200 samples to guarantee rapid execution latency later during MLE training.
%
And (iv) \textit{Concrete Specification Compilation}: the agent merges these elements, defining a complex hidden rule $H: l = f(z) + \epsilon$ that connects individual features $z$ to labels $l$ in the synthetic micro dataset $Z$.
%
For instance, in an urban road damage detection task, the rule might dictate that a specific edge pixel ratio ($f(z)$) combined with injected blur noise ($\epsilon$) strictly determines the final damage severity label ($l$). 
%
The agent simultaneously restricts the total dataset size to 50--200 samples to guarantee rapid execution latency later during MLE training.
%
To mitigate the challenge of sparse reward signals in later policy optimization, the agent also specifies multiple baseline methods of varying complexity. 
%
These methods theoretically establish a set of progressive milestone thresholds $\mathcal{S}$ to enable dense reward assignment.
%


\paragraph{ML Developer: Synthetic Data Generation.}
\label{subsec:agentic_data_generation}
To translate these abstract specifications into executable environments, an \textit{ML Developer} agent writes a self-contained Python script to perform four critical operations.
%
First, it synthesizes the micro-scale datasets $Z$ and partitions them into training ($\mathcal{D}_{\text{train}}$) and hidden test ($\mathcal{D}_{\text{test}}$) sets. 
%
Then, it implements the defined hidden rules $H$ to deterministically map the generated features $z$ to ground-truth labels $l$ via $H: l = f(z) + \epsilon$.
%
Continuing our previous example of road damage detection task, the agent writes the procedural code to generate the synthetic urban road images, calculates the edge pixel ratio $f(z)$ for each, injects the specified blur noise $\epsilon$, and mathematically assigns the final damage severity label $l$.
% \zz{connecting to the previous paragraph, maybe it is better to continue the example? previous paragraph is to define, here is to implement, right?}
%
Next, the script trains and evaluates the \textit{Data Strategist}'s specified baseline methods to empirically calculate and lock in the set of progressive milestone thresholds $\mathcal{S}$ required for downstream dense reward calculation.
%
Finally, it outputs a dummy sample submission file containing the test data paired with random predictions to serve as a strict schema reference. 
%
To ensure environment reliability, we enforce an \textit{execution-based verification loop}: if the script fails, the current trace is automatically returned to the agent for iterative debugging.
% \zz{is this detail important to the method itself?}
%


\paragraph{MLOps Engineer: Evaluation Environment Setup.}
% \zz{An MLOps Engineer bridges data science and operations, automating the deployment, monitoring, and management of machine learning models in production.}
\label{subsec:eval_environment}
To construct the automated scoring sandbox, an \textit{MLOps Engineer} agent writes a robust \texttt{evaluator script} based on the task specification and training data $\mathcal{D}_{\text{train}}$. 
%
This process involves three key requirements: 
First, \textit{metric standardization}: the agent hard-codes the evaluation metric $\mathcal{M}$, the optimization direction, and the set of progressive milestone thresholds $\mathcal{S}$ to ensure deterministic scoring.
%
Second, \textit{data alignment and computation}: the script loads an agent's submission (containing predictions $\hat{p}$), aligns it with the hidden ground truth labels $l \in \mathcal{D}_{\text{test}}$, computes the exact metric $\mathcal{M}(\hat{p}, l)$, and outputs the final score. 
%
And third, \textit{execution-based verification}: to guarantee reliability, the system automatically tests the \texttt{evaluator script} against a dummy sample submission.
% \zz{define dummy sample submission? is it the most basic baseline that gets up to $s_1$?}
%
Any runtime errors are fed back to the \textit{MLOps Engineer} for iterative debugging to finalize a functional evaluation environment.
%
As a final quality gate, the pipeline verifies that the milestone thresholds satisfy strict monotonic ordering consistent with the metric's optimization direction, discarding tasks that fail this constraint (details in \appref{sec:sanity}).
%

\paragraph{Technical Writer: Task Description Synthesis.}
\label{subsec:task_description}
Once data and environments are generated, a \textit{Technical Writer} agent compiles metadata into a markdown document (\secref{subsec:task_description}).
%
This synthesis involves: 
(i) \textit{contextual integration}, adapting the original task’s narrative to the synthetic domain;
(ii) \textit{content generation}, drafting the problem overview and evaluation metrics; 
(iii) \textit{submission formatting}, defining the output schema; and (iv) \textit{file transparency}, cataloging public data while omitting hidden test data. 
%
This documentation pipeline ensures the final synthetic task prompt, which serves as the initial task specification $\mathcal{I}$ as in \secref{subsec:SDP}, is realistic and perfectly aligned with the evaluation code. 
%
% Further task verification details and agent prompt templates are provided in \appref{sec:sanity} and \appref{sec:prompt}, respectively.
%

\subsection{Trajectory-Level GRPO}\label{subsec:trajectory_grpo}
\paragraph{Enable On-policy RL for MLE Tasks.}
While trajectory-level GRPO has proven effective for SWE and web search tasks~\citep{deepswe2025, wu2025webdancer}, applying it to MLE tasks has remained computationally infeasible.
%
The synthetic micro-scale environments constructed by our pipeline (\secref{subsec:synthetic_pipeline}) reduce the wall-clock cost and transforms trajectory-level GRPO from a theoretical possibility into a practical training paradigm for MLE agents.
%

Concretely, during the rollout phase, the LLM agent interacts with a \ours environment using the ReAct framework~\citep{yao2022react}.
%
Starting from the initial task specification $\mathcal{I}$, the agent iteratively generates actions (code or reasoning) and receives observations (execution output, errors, or intermediate metrics) over multiple turns using the available tool set $\mathcal{T}$.
%
To ensure computational efficiency, we enforce strict boundary conditions on the environment: a per-step execution time limit $\tau_{\max}$ and a maximum trajectory length $T_{\max}$. 
%
The agent's trajectory terminates when it yields a final submission or reaches $T_{\max}$.
%

\paragraph{Dense Reward Formulation.}
In complex agentic tasks, relying solely on the final performance metric often results in a sparse reward signal, making policy optimization highly unstable. 
%
To mitigate this sparsity, we design a dense reward function composed of two primary components: a \textit{format reward} and a \textit{milestone-based reward}. 
%
The final verifiable reward $r$ provides granular feedback across the entire trajectory and is defined as follows:
%
$
    r = w_{\text{format}} \cdot r_{\text{format}} + w_{\text{execute}} \cdot \mathbb{I}_{\text{execute}} + \sum_{i=1}^{k} w_{S_i} \cdot \mathbb{I}_{S_i}.
$
%
Here, the format reward $r_{\text{format}} \in [0, 1]$ represents the ratio of generated steps that properly utilize the required \texttt{<think>...</think>} reasoning tags. 
%
The milestone-based component evaluates the final state of the environment using boolean indicator functions ($\mathbb{I} \in \{0, 1\}$). 
%
This includes basic execution milestones---such as successfully generating and formatting a valid output file ($\mathbb{I}_{\text{execute}}$)---as well as tiered performance milestones ($\mathbb{I}_{S_i}$) that evaluate whether the final quantitative score surpasses the predefined thresholds in our progressive set $\mathcal{S}$. 
%
By distributing fixed weights ($w$) across these terms to sum to a maximum of $1.0$, this milestone-based reward smoothly guides the agent from basic formatting compliance and code execution to state-of-the-art performance. More details of GRPO training design can be found in \appref{sec:mask}
% \zz{The last sentence implies that $w$ changes during training (so that it guides the focus from formatting to performance), is this intended?}
%


==> colm_sections/5_experiments.tex <==
\section{Experiments}\label{sec:experiments}
% We design our experiments to rigorously evaluate the effectiveness of both the synthetic dataset and the GRPO training framework.

\subsection{Experimental Setup}
\paragraph{Dataset.}
We construct our training corpus \textit{seeded} from the MLE-bench dataset~\citep{chan2024mle}.
%
Specifically, we collect 60 questions spanning the \texttt{Medium}, \texttt{Hard}, and \texttt{Dev} splits as seeds to ensure exposure to diverse reasoning patterns.
%
% These seeds undergo domain mutation and difficulty boosting, followed by automated sanity check to filter for resolvability and schema validity, as discussed in \secref{sec:workflow}. 
%
This process yields a final training dataset of 848 synthetic tasks for training and 64 held-out tasks for validation (filtering process in \appref{sec:filtering}). 
%
To evaluate real-world generalization, we employ two benchmarks: MLE-bench-lite, comprising unseen questions from the \texttt{Easy} split, and MLE-Dojo~\citep{qiang2025mle}, a curated collection of 62 additional tasks from broader Kaggle competitions.
%

\paragraph{Evaluation Metrics.}
Following the evaluation protocol established by MLE-bench~\citep{chan2024mle}, we measure performance using a hierarchy of success metrics: \texttt{Valid Submission}, \texttt{Above Median}, \texttt{Bronze}, \texttt{Silver}, \texttt{Gold}, and \texttt{Any Medal}. 
%
These Kaggle-style tiers serves as the concrete instantiation of the abstract progressive milestone set $\mathcal{S} = \{s_1, s_2, \dots, s_k\} = \{s_\text{median}, s_\text{bronze}, s_\text{silver}, s_\text{gold}\}$ introduced in \secref{subsec:synthetic_pipeline}, with each tier corresponding to a progressively more demanding leaderboard percentile.
%
Among these, \texttt{Any Medal} (the union of \texttt{Bronze}, \texttt{Silver}, and \texttt{Gold}) serves as our primary metric.
%
For MLE-Dojo~\citep{qiang2025mle}, we adhere to the original setup by reporting the \texttt{Valid Submission} rate and the \texttt{HumanRank Score}.
%
More detailed definitions for all metrics are provided in \appref{sec:metric_definition_details}.
%

\paragraph{Agent Scaffolds.}
Recognizing that model performance is heavily influenced by the choice of agentic scaffolding, we evaluate models across a diverse set of agent frameworks to demonstrate their generalization capabilities.
% \zz{We need to update this since in main results we only have react right?}
%
For MLE-bench-lite, we employ ReAct (consistent with our GRPO rollout)~\citep{yao2022react}, AIRA~\citep{toledo2025ai}, and AIDE~\citep{jiang2025aide}. 
%
For MLE-Dojo benchmark, we employ its native MLE Agent scaffold~\citep{qiang2025mle} and AIDE, ensuring a robust assessment of our model's adaptability to different agent architectures.
%

\paragraph{Models and Baselines.}
We apply the proposed \ours training pipeline to three LLMs with varying size: \texttt{Qwen3-8B}, \texttt{Qwen3-14B} and \texttt{Qwen3-30B-A3B-2507}~\citep{yang2025qwen3}. 
%
\texttt{Seed-SFT} is a SFT baseline designed to disentangle the benefit of seed data from RL: we prompt Claude-4.5-Sonnet~\citep{anthropic2025sonnet45} to generate reasoning trajectories for the 60 seed questions used in our synthetic generation pipeline, then finetune the base model on these interactions via standard SFT.
%
And \texttt{\ours} denotes models finetuned via trajectory-wise GRPO on our synthetic corpus, starting from the \texttt{Base} checkpoint.
%
\texttt{SFT-\ours} applies the same GRPO training but initializes from the Seed-SFT checkpoint, allowing us to assess whether SFT and RL provide complementary benefits.
%
We also report the performance of Claude-4.5-Sonnet, DeepSeek-V3.1~\citep{liu2024deepseek}, and Gemini-2.5-Flash~\citep{huang2025gemini} as reference points from models that are orders of magnitude larger.
% For our proposed method, we denote the models finetuned via GRPO on the synthetic corpus as \textbf{\ours}. 
%
% To isolate the benefits of RL finetuning from SFT on high-quality seed data, we also compare against a strong baseline, \textbf{Seed-SFT}. This baseline is obtained by first prompting Claude-4.5-Sonnet~\citep{anthropic2025sonnet45} to generate reasoning trajectories for the 60 seed questions used in our synthetic generation pipeline, and then fine-tuning the base models on these multi-turn interactions using standard SFT. Additionally, we report the performance of Claude-4.5-Sonnet, Deepseek-V3.1 and Gemini-2.5-flash~\citep{huang2025gemini, liu2024deepseek} to serve as upper bound reference points.


\paragraph{Implementation Details.}
Given the milestone-to-tier mapping above, we assign the specific reward weights in our reward formulation \secref{subsec:trajectory_grpo} as follows: $w_{\text{format}} = 0.1$, $w_{\text{execute}} = 0.2$, $w_{s_\text{median}} = 0.1$, $w_{s_\text{bronze}} = 0.2$, $w_{s_\text{silver}} = 0.2$, and $w_{s_\text{gold}} = 0.2$. 
%
We restrict $T_{\max} = 20$ and $\tau_{\max} = 90$ seconds.
%
More hyperparameter details can be found in \appref{sec:hyperparameter}.
%

\subsection{Statistics of Synthetic Training Data}
\label{sec:statistics}
\paragraph{Domain, Modality, and Tasks.}
% Detailed in \appref{sec:domain}, the diverse domain, modality, and task distributions of our synthetic data underscore the amplification capacity of the \texttt{Data Strategist} agent (\secref{subsec:synthetic_pipeline}).
From only 60 seed tasks, our pipeline generates a corpus spanning 8+ application domains (e.g., healthcare, retail, manufacturing), 6 data modalities (image, tabular, text, multi-modal, graph, audio), and diverse task formulations including classification, regression, and ranking. 
%
Full distributions are provided in \appref{sec:domain}.
%


\paragraph{Task Reliability and Difficulty Calibration.}
\begin{wrapfigure}{r}{0.45\textwidth}
\vspace{-0.1in}
    \centering
    % \includegraphics[width=\linewidth]{figure/model_reward_heatmap.pdf}
    \includegraphics[width=\linewidth]{figure/model_wins_combined.pdf}
    \vspace{-0.25in}
    \caption{
        Pairwise win counts and win rates (\%) across 64 synthetic tasks. 
        %
    }
    \label{fig:model_pairwise}
    \vspace{-0.22in}
\end{wrapfigure}
To validate that our synthetic tasks are both non-trivial and properly calibrated in difficulty, we benchmark four models with well-established capability differences: \texttt{GPT-4o-mini}~\citep{hurst2024gpt}, \texttt{Gemini-2.5-Flash}~\citep{huang2025gemini}, \texttt{DeepSeek-V3}~\citep{guo2025deepseek}, and \texttt{Claude-4.5-Sonnet}.
We randomly sample 64 tasks from our synthetic corpus and compare model performances pairwise, assigning 1 point for a win, 0 for a loss, and 0.5 for a tie.
%
% As shown in \figref{fig:model_pairwise}, the aggregated win counts reproduce the expected capability ordering: Claude-4.5 dominates with a 92.9\% win rate, followed by DeepSeek-V3 (39.9\%), Gemini-2.5 (35.6\%), and GPT-4o-mini (25.5\%).
As shown in \figref{fig:model_pairwise}, the aggregated win counts reproduce the expected capability ordering.
%
The fact that our tasks cleanly separate models of known capability confirms that they capture meaningful MLE task difficulty and are sufficiently challenging to serve as a training signal.
%


\paragraph{Dataset Scale and Execution Latency.}
Each synthetic task generated by our pipeline comes with an associated training dataset that the agent's ML pipeline must process during rollouts.
%
% \begin{wrapfigure}{r}{0.45\textwidth}
% \vspace{-0.37in}
%     \centering
%     \includegraphics[width=\linewidth]{figure/exec_time_dumbbell.pdf}
%     \vspace{-0.25in}
%     \caption{
%         Avg. code execution time on original MLE-bench seed tasks versus \ours synthetic tasks.
%     }
%     \label{fig:time_comp}
%     \vspace{-0.2in}
% \end{wrapfigure}
The size of this per-task dataset directly determines code execution latency and is therefore the key lever for making on-policy RL feasible.
%
For context, the original 60 seed tasks from MLE-bench contain an average of approximately 4.09 million samples per task~\citep{chan2024mle}, making each rollout step prohibitively slow. 
%
By contrast, our pipeline intentionally constrains the per-task dataset to a micro-scale regime: as shown in \figref{fig:data_size_distribution} in \appref{sec:qualitative_analysis}, the majority of tasks contain between 120 and 150 samples each.
%
\begin{wrapfigure}{r}{0.45\textwidth}
\vspace{-0.2in}
    \centering
    \includegraphics[width=\linewidth]{figure/exec_time_dumbbell.pdf}
    \vspace{-0.25in}
    \caption{
        Avg. code execution time on original MLE-bench seed tasks versus \ours synthetic tasks.
    }
    \label{fig:time_comp}
    \vspace{-0.2in}
\end{wrapfigure}
%

The impact on execution latency is dramatic.
%
Using code implementations generated by \texttt{Gemini-2.5-Flash}, the average execution time drops from 196.17 seconds on the original MLE-bench tasks to just 14.31 seconds on our synthetic tasks, a reduction of over $13\times$, as shown in \figref{fig:time_comp}.
%
This speedup is what transforms trajectory-wise GRPO from infeasible to practical, enabling thousands of on-policy rollout updates in the wall-clock time previously consumed by a handful of steps on the original benchmark.
%
A comprehensive qualitative analysis of a representative generated task is also provided in \appref{sec:quality}.
%


\subsection{Main Results}\label{sec:main_results}
% To evaluate the effectiveness of our proposed approach, we first benchmark our method against baselines on the MLE-bench-lite dataset using the standard ReAct framework (consistent with our GRPO rollouts).

\paragraph{Comparison with Baselines.}
As shown in \tabref{tab:main_results}, \texttt{\ours} achieves significant gains at every scale: +66.9\% relative improvement on \texttt{Any Medal} rate at 8B, +24.7\% at 14B, and +100.7\% at 30B over their respective \texttt{Base} models. 
%
By comparison, the off-the-shelf \texttt{Base} models achieve between 13.6\% and 18.2\% \texttt{Any Medal} rate, and the \texttt{Seed-SFT} baseline---despite leveraging 60 high-quality \texttt{Claude-4.5-Sonnet} trajectories---yields marginal or zero improvement over \texttt{Base} (e.g., \texttt{Any Medal} rate remains at 13.6\% for both 8B and 30B). In contrast, our \texttt{\ours} achieves a substantial 20.3\% to 66.9\% relative improvement over the \texttt{Seed-SFT} baseline.
%
This gap suggests that behavioral cloning on expert trajectories does not transfer the iterative problem-solving behavior that trajectory-wise RL acquires through direct environment interaction.
%
Moreover, these RL-driven improvements propel our open-weight models to rival closed-source systems; our 8B \texttt{\ours} matches the 22.7\% \texttt{Any Medal} rate of Deepseek-V3.1 and Gemini-2.5-flash, while our 14B and 30B models (27.3\%) aggressively close the gap with the top-performing Claude-4.5-Sonnet (31.8\%).

\paragraph{Combining SFT and RL.}
Initializing GRPO from the \texttt{Seed-SFT} checkpoint (\texttt{SFT-\ours}) consistently improves operational reliability without sacrificing \texttt{Any Medal} rate. 
%
as shown in \tabref{tab:main_results}, at 8B, \texttt{SFT-\ours} raises \texttt{Valid Submission} to 90.9\% while maintaining 22.7\% \texttt{Any Medal} rate.
%
At 14B, this variant achieves 95.5\% \texttt{Valid Submission} and 27.3\% \texttt{Any Medal}. 
%
These results indicate that SFT and RL contribute along different axes---format compliance from SFT, higher-order reasoning from RL---and combine effectively.
%

\paragraph{Scaling with Model Sizes.}
Scaling model capacity yields improvements along multiple axes. 
%
Most visibly, \texttt{Valid Submission} for pure \texttt{\ours} increases monotonically from 63.6\% to 100\%, while the \texttt{Base} models remain flat at 68--73\% across scales. 
%
% This suggests that, at smaller scales, the RL policy explores aggressive strategies that do not always produce valid outputs, and that sufficient model capacity resolves this tension between exploration and output reliability. 
%
Beyond submission validity, \texttt{Above Median} rate for \texttt{\ours} also scales from 27.3\% (8B) to 36.4\% (30B), compared to a static 18.2\% for all \texttt{Base} models, indicating that the gains are not limited to a few tasks but reflect broadly improved engineering competence. 
%
Finally, the reliance on SFT initialization diminishes with scale: the \texttt{Valid Submission} gap between \texttt{\ours} and \texttt{SFT-\ours} narrows from 27.3\% at 8B to 18.2\% at 14B, and inverts at 30B where pure \texttt{\ours} achieves 100\% without SFT. 
%
This suggests that larger models can internalize both the formatting discipline and the reasoning capability through RL alone.
%
Additionally, we conduct an ablation study of our reward design in Appendix \ref{sec:ablation_reward}, which demonstrates the effectiveness of our milestone-based reward in enabling these optimizations.



% \textit{Our \ours approach yields substantial performance improvements across all model scales, rendering open-weight models highly competitive with proprietary systems.} 
% The empirical results in \tabref{tab:main_react_results} demonstrate the clear efficacy of our proposed synthetic RL finetuning approach. 
% %
% Advanced, closed-source models—namely Claude-4.5-Sonnet, Deepseek-V3.1, and Gemini-2.5-flash—establish strong upper-bound reference points for this benchmark.
% %
% Conversely, the open-weight Base models naturally struggle out-of-the-box with complex, multi-step engineering tasks. 
% %
% Crucially, we observe that the Seed-SFT baseline, which utilizes behavioral cloning on the 60 high-quality seed trajectories, frequently yields marginal improvements or even degrades performance compared to the Base model.
% %

% In contrast, our RL-finetuned variants (both pure \ours and SFT-\ours) consistently outperform both the Base and SFT baselines, aggressively closing the gap with state-of-the-art closed-source models. 
% %
% Strikingly, at the 8B scale, both Qwen3-8B-\ours and Qwen3-8B-SFT-\ours achieve a 22.7\% \texttt{Any Medal} rate, noticeably surpassing the SFT baseline of 13.6\% and directly matching the "Any Medal" performance of both Deepseek-V3.1 and Gemini-2.5-flash. 
% %
% Furthermore, the SFT-\ours variant demonstrates exceptional stability, achieving a 90.9\% Valid Submission rate.

% This strong scaling trend continues and amplifies when combining SFT with our RL pipeline. The Qwen3-14B-SFT-\ours model achieves a remarkable 27.3\% Any \texttt{Any Medal} rate and a 95.5\% Valid Submission rate, securing the top spot in almost every category for its scale. At the 30B scale, both RL-driven variants definitively outperform Deepseek-V3.1 and Gemini-2.5-flash. The pure Qwen3-30B-\ours model achieves an impressive 27.3\% \texttt{Any Medal} rate with a perfect 100\% valid submission rate, while the Qwen3-30B-SFT-\ours model matches this 27.3\% \texttt{Any Medal} rate and achieves the highest "Above Median" score (45.5\%) across all 30B configurations. This demonstrates that applying our synthetic RL pipeline on top of the Seed-SFT checkpoint offers complementary benefits across all model sizes, bringing the 30B and 14B open-weight models to a highly competitive level with the top-performing Claude-4.5-Sonnet (31.8\% Any Medal). Ultimately, this confirms that optimizing via trajectory-wise reinforcement learning on procedural synthetic environments successfully instills genuine, transferable engineering reasoning that rivals much larger, proprietary systems.

\begin{table}[tb]
\centering
\caption{
    Main results on the MLE-bench-lite dataset using the ReAct framework. 
    %
    \texttt{\ours} refers to model finetuned through our proposed pipeline.
    %
}
\vspace{-0.1in}
\label{tab:main_results}
\setlength{\tabcolsep}{8pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l cccccc}
\toprule
\textbf{Model} & \textbf{Valid Sub.} & \textbf{Above Median} & \textbf{Bronze} & \textbf{Silver} & \textbf{Gold} & \textbf{Any Medal} \\
\midrule
Deepseek-V3.1 & 90.9 & 36.4 & 0.0 & 4.5 & 18.2 & 22.7 \\
Gemini-2.5-flash & 81.8 & 45.5 & 4.5 & 4.5 & 13.6 & 22.7 \\
Claude-4.5-Sonnet & 95.5 & 31.8 & 0.0 & 4.5 & 27.3 & 31.8 \\
\midrule
\multicolumn{7}{c}{\textbf{Qwen3-8B}} \\
\midrule
Qwen3-8B-Base & 68.2 & 18.2 & 0.0 & 4.5 & 9.1 & 13.6 \\
Qwen3-8B-Seed-SFT & 72.7 & 18.2 & \textbf{4.5} & 0.0 & 9.1 & 13.6 \\
Qwen3-8B-\ours & 63.6 & 27.3 & 0.0 & \textbf{4.5} & \textbf{18.2} & \textbf{22.7} \\
Qwen3-8B-SFT-\ours & \textbf{90.9} & \textbf{31.8} & \textbf{4.5} & 0.0 & \textbf{18.2} & \textbf{22.7} \\
\midrule
\multicolumn{7}{c}{\textbf{Qwen3-14B}} \\
\midrule
Qwen3-14B-Base & 72.7 & 18.2 & 4.5 & 4.5 & 18.2 & 18.2 \\
Qwen3-14B-Seed-SFT & 72.7 & 22.7 & 4.5 & 0.0 & 13.6 & 18.2 \\
Qwen3-14B-\ours & 77.3 & 27.3 & \textbf{4.5} & \textbf{4.5} & 13.6 & 22.7 \\
Qwen3-14B-SFT-\ours & \textbf{95.5} & \textbf{31.8} & \textbf{4.5} & 0.0 & \textbf{22.7} & \textbf{27.3} \\
\midrule
\multicolumn{7}{c}{\textbf{Qwen3-30B-A3B}} \\
\midrule
Qwen3-30B-Base & 68.2 & 18.2 & 4.5 & 0.0 & 9.1 & 13.6 \\
Qwen3-30B-Seed-SFT & 77.3 & 31.8 & 4.5 & 4.5 & 13.6 & 22.7 \\
Qwen3-30B-\ours & \textbf{100.0} & 36.4 & 0.0 & \textbf{13.6} & \textbf{13.6} & \textbf{27.3} \\
Qwen3-30B-SFT-\ours & 90.9 & \textbf{45.5} & \textbf{4.5} & 9.1 & \textbf{13.6} & \textbf{27.3} \\
\bottomrule
\end{tabular}
}
\vspace{-0.1in}
\end{table}



% \subsection{Test-Time Scaling of \ours Models}\label{sec:test_time_scaling}
% To further understand the behavior of our model trained via \ours, we investigate test-time scaling by varying the maximum allowed interaction turns $T_{\max}$ for the \texttt{Qwen3-30B-SFT-\ours} model within the ReAct framework.
% %
% For these experiments, the maximum compute limit is fixed at 24 GPU hours per task. 
% %
% As the number of iterations $T_{\max}$ grows, the agent's trajectory naturally risks exceeding the context window of the \texttt{Qwen3} model.
% %
% To mitigate this, we employ a dynamic truncation strategy: if the context window limit is reached, we systematically remove older messages that contain failed code executions to free up context space. 
% %

% %
% As shown in \figref{fig:test_time_scaling}, the model exhibits clear positive test-time scaling, successfully sustaining self-improvement abilities as it is granted more turns to iterate. 
% %
% This sustained scaling demonstrates the effectiveness of our \ours approach in instilling robust trial-and-error reasoning. 
% %
% Both \texttt{Any Medal} and \texttt{Above Median} rates increase steadily, peaking at a limit of 30 turns. 
% %
% However, scaling beyond this threshold causes a performance regression due to frequent context window overflows. 
% %
% Despite our message eviction strategy, the sheer loss of historical context disrupts the agent's long-horizon memory, often trapping it in repetitive loops. 
% %
% This highlights that test-time scaling in complex MLE tasks is ultimately bottlenecked by the model's effective context length.
% %


\paragraph{Training Dynamics.}
We track training and validation rewards across various models over GRPO steps (details and full curves in \appref{app:training_dynamics}).
%
We observe that the RL objective converges stably on our synthetic environments across all scales, validating that the synthetic tasks provide a sufficiently diverse and well-calibrated training signal.
% %
% Larger models both start higher and converge to higher reward ceilings, consistent with the evaluation-time scaling trends as shown in \tabref{tab:main_results}.
% %
% Notably, the ability to produce valid submissions is itself a learned behavior: smaller models acquire it slowly and inconsistently during training, while the bigger 30B model internalizes it early and maintains it throughout, explaining why pure \texttt{Qwen3-30B-\ours} no longer requires SFT initialization for output reliability.
% %

\paragraph{Test-Time Scaling.}
% Furthermore, we investigate test-time scaling by varying the maximum allowed interaction turns $T_{\max}$ for the \texttt{Qwen3-30B-SFT-\ours} model within the ReAct framework, as detailed in \appref{sec:test_time_scaling}. We observe that the model exhibits clear positive test-time scaling. This sustained scaling demonstrates the effectiveness of our \ours approach in instilling robust trial-and-error reasoning. 
We vary the maximum interaction turns $T_{\max}$ for \texttt{Qwen3-30B-SFT-\ours} under ReAct (details and full curves in \appref{sec:test_time_scaling}).
%
Any Medal rate climbs from 5\% at 5 turns to 55\% at 30 turns, confirming that \ours instills robust trial-and-error reasoning. 
%
Beyond 30 turns, performance regresses as context window overflows force eviction of earlier history, suggesting that effective context length is the current bottleneck for further test-time scaling.







==> colm_sections/6_analysis.tex <==
\begin{table}[t]
\centering
\caption{Generalization results on the MLE-bench-lite across alternative agent frameworks.}
\vspace{-0.1in}
\label{tab:generalization_lite}
\setlength{\tabcolsep}{6pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ll cccccc}
\toprule
\textbf{Model} & \textbf{Framework} & \textbf{Valid Sub.} & \textbf{Above Med.} & \textbf{Bronze} & \textbf{Silver} & \textbf{Gold} & \textbf{Any Medal} \\
\midrule
\multicolumn{8}{c}{\textbf{Qwen3-14B}} \\
\midrule
% Qwen3-14B-Base & ML-Master & 27.3 & 4.5 & 0.0 & 0.0 & 4.5 & 4.5 \\
% \cmidrule{1-8}
Qwen3-14B-Base & AIDE & 100.0 & 36.4 & 0.0 & 4.5 & \textbf{22.7} & 27.3 \\
Qwen3-14B-Seed-SFT & AIDE & 100.0 & 31.8 & 0.0 & 9.1 & 9.1 & 18.2 \\
Qwen3-14B-\ours & AIDE & \textbf{100.0} & \textbf{40.9} & 0.0 & \textbf{13.6} & 18.2 & \textbf{31.8} \\
\cmidrule{1-8}
Qwen3-14B-Base & AIRA & 100.0 & 22.7 & 0.0 & 0.0 & 9.1 & 9.1 \\
Qwen3-14B-Seed-SFT & AIRA & 95.5 & 22.7 & 0.0 & 0.0 & 13.6 & 13.6 \\
Qwen3-14B-\ours & AIRA & \textbf{100.0} & \textbf{36.4} & \textbf{4.5} & 0.0 & \textbf{18.2} & \textbf{22.7} \\
\midrule
\multicolumn{8}{c}{\textbf{Qwen3-30B-A3B}} \\
\midrule
Qwen3-30B-Base & AIDE & 95.5 & 18.2 & 4.5 & 0.0 & 9.1 & 13.6 \\
Qwen3-30B-Seed-SFT & AIDE & 100.0 & 18.2 & 4.5 & 0.0 & \textbf{9.1} & 13.6 \\
Qwen3-30B-\ours & AIDE & \textbf{100.0} & \textbf{18.2} & \textbf{9.1} & \textbf{0.0} & 4.5 & \textbf{13.6} \\
\cmidrule{1-8}
Qwen3-30B-Base & AIRA & 86.4 & 27.3 & 0.0 & 0.0 & 18.2 & 18.2 \\
Qwen3-30B-Seed-SFT & AIRA & 100.0 & 22.7 & 0.0 & \textbf{4.5} & 9.1 & 13.6 \\
Qwen3-30B-\ours & AIRA & \textbf{100.0} & \textbf{40.9} & \textbf{4.5} & 0.0 & \textbf{22.7} & \textbf{27.3} \\
\bottomrule
\end{tabular}
}
\vspace{-0.1in}
\end{table}
%
\section{Analysis and Framework Generalization}\label{sec:generalization}
%
As model performance on MLE tasks is sensitive to the choice of agent scaffold, we evaluate the 14B and 30B models across alternative frameworks---AIDE~\citep{jiang2025aide} and AIRA~\citep{toledo2025ai} on MLE-bench-lite (\tabref{tab:generalization_lite}), and AIDE~\citep{jiang2025aide} and MLE-Agent~\citep{qiang2025mle} on MLE-Dojo (\tabref{tab:generalization_dojo})---to assess whether the gains from \texttt{\ours} transfer beyond the ReAct scaffold used in training.
\begin{wraptable}{r}{0.5\textwidth}
% \begin{table}[t]
% \vspace{-0.1in}
\centering
\caption{
    Generalization results on the MLE-Dojo benchmark. 
    %
    The HumanRank Score measures relative leaderboard performance against human competitors. 
    %
    % Only 14B and 30B models are shown.
}
\vspace{-0.1in}
\label{tab:generalization_dojo}
\setlength{\tabcolsep}{2pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{ll cc}
\toprule
\textbf{Model} & \textbf{Framework} & \textbf{Valid Sub. (\%)} & \textbf{HumanRank} \\
\midrule
Claude-4.5-Sonnet & MLE-Agent & 91.9 & 54.09 \\
\midrule
\multicolumn{4}{c}{\textbf{Qwen3-14B}} \\
\midrule
Qwen3-14B-Base & MLE-Agent & 27.4 & 9.62 \\
Qwen3-14B-Seed-SFT & MLE-Agent & 3.2 & 0.65 \\
Qwen3-14B-\ours & MLE-Agent & \textbf{40.3} & \textbf{12.55} \\
\cmidrule{1-4}
Qwen3-14B-Base & AIDE & 74.2 & 37.73 \\
Qwen3-14B-Seed-SFT & AIDE & 62.9 & 27.51 \\
Qwen3-14B-\ours & AIDE & \textbf{75.8} & \textbf{37.86} \\
\midrule
\multicolumn{4}{c}{\textbf{Qwen3-30B-A3B}} \\
\midrule
Qwen3-30B-Base & MLE-Agent & 71.0 & 29.12 \\
Qwen3-30B-Seed-SFT & MLE-Agent & 17.7 & 7.34 \\
Qwen3-30B-\ours & MLE-Agent & \textbf{83.9} & \textbf{38.56} \\
\cmidrule{1-4}
Qwen3-30B-Base & AIDE & 59.7 & 25.99 \\
Qwen3-30B-Seed-SFT & AIDE & 66.1 & 28.14 \\
Qwen3-30B-\ours & AIDE & \textbf{77.4} & \textbf{28.72} \\
\bottomrule
\end{tabular}
}
% \end{table}
\vspace{-0.1in}
\end{wraptable}
% 
% Because model performance in machine learning tasks is highly sensitive to the chosen agentic scaffold, we evaluated the larger capacity models (14B and 30B) across alternative frameworks, including AIDE, AIRA, MLE-Agent, and ML-Master, to test algorithmic robustness. 
% \paragraph{Framework-agnostic Generalization.}
As shown in \tabref{tab:generalization_lite} (for MLE-bench-lite) and \tabref{tab:generalization_dojo} (for MLE-Dojo), 
\ours consistently exceeds \texttt{Base} model performance across all scaffold-benchmark combinations.
%
While the SFT models prove brittle when deployed outside the specific scaffold used during their data generation, most notably collapsing to a 17.7\% \texttt{Valid Submission} rate on MLE-Dojo for the 30B model with MLE-Agent, the \ours models adapt robustly. 
%
Specifically, on the MLE-Dojo benchmark, Qwen3-30B-\ours paired with MLE-Agent framework achieves an 83.9\% \texttt{Valid Submission} rate and a HumanRank score of 38.56, vastly outperforming both the Base and SFT variants. We observe similar robustness on MLE-bench-lite, where the 14B and 30B \ours models consistently elevate the \texttt{Any Medal} and \texttt{Valid Submission} rate across AIDE and AIRA scaffolds. 
% It is also worth noting the anomalous underperformance observed when utilizing the ML-Master framework (Table \ref{tab:generalization_lite}); due to its specific memory management approach, the framework frequently causes out-of-context window overflows for the Qwen3 models, leading to severe performance regression regardless of the underlying model reasoning capabilities.



==> colm_sections/7_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this work, we introduced \ours, a framework that makes trajectory-wise on-policy RL practical for MLE agents by generating diverse, verifiable synthetic environments with micro-scale datasets.
%
Our approach is grounded in the observation that MLE latency is overwhelmingly driven by the size of the datasets that each ML pipeline must process during training and inference.
%
By constructing tasks from the ground up at 50--200 samples, we reduce per-step execution time by over 13$\times$ while preserving the structural complexity needed for meaningful policy optimization.
%
Combined with a dense, milestone-based reward formulation, this enables stable GRPO training that yields 20.3\% to 66.9\% relative improvement in medal rate over the SFT baseline across model scales on MLE-bench-lite, and generalizes robustly across unseen agentic scaffolds.
%
We believe the principle underlying \ours---that synthetic micro-scale environments can serve as effective proxies for real-world MLE tasks---opens a scalable path toward training MLE agents that improve through direct environment interaction rather than imitation of expert behavior.
%


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}



% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

